Discrimination through Image Selection by Job Advertisers on Facebook

Targeted advertising platforms are widely used by job advertisers to reach potential employees; thus issues of discrimination due to targeting that have surfaced have received widespread attention. Advertisers could misuse targeting tools to exclude people based on gender, race, location and other protected attributes from seeing their job ads. In response to legal actions, Facebook disabled the ability for explicit targeting based on many attributes for some ad categories, including employment. Although this is a step in the right direction, prior work has shown that discrimination can take place not just due to the explicit targeting tools of the platforms, but also due to the impact of the biased ad delivery algorithm. Thus, one must look at the potential for discrimination more broadly, and not merely through the lens of the explicit targeting tools. In this work, we propose and investigate the prevalence of a new means for discrimination in job advertising, that combines both targeting and delivery -- through the disproportionate representation or exclusion of people of certain demographics in job ad images. We use the Facebook Ad Library to demonstrate the prevalence of this practice through: (1) evidence of advertisers running many campaigns using ad images of people of only one perceived gender, (2) systematic analysis for gender representation in all current ad campaigns for truck drivers and nurses, (3) longitudinal analysis of ad campaign image use by gender and race for select advertisers. After establishing that the discrimination resulting from a selective choice of people in job ad images, combined with algorithmic amplification of skews by the ad delivery algorithm, is of immediate concern, we discuss approaches and challenges for addressing it.

==> tables/truck_nurse_percentage.tex <==
\begin{table}[htb]
\caption{ Percentage of Advertisers Who Exclusively Use People of Stereotypical Gender in Their Images. We consider all advertisers whose campaigns contain at least one image with people.
\ak{ I think what this table is really missing is another multicolumn for Number of Distinct People-Containing Images and Statistics for those}
\varun{add the statistic for >=15}
\varun{turns out we don't have advertisers with >=15 distinct people-containing images and exclusively use men/women}
}
\label{tab:truck_nurse_selective_perc}
\resizebox{\textwidth}{!}{\begin{tabular}{l|c|ccccc|ccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Statistic}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Across All Advertisers \\ With $\geq 1$ Image\end{tabular}}} &
  \multicolumn{5}{c|}{\textbf{Number of Images}} &
  \multicolumn{5}{c}{\textbf{Number of Distinct Images}} \\ \cline{3-12} 
\multicolumn{1}{c|}{} &
   &
  \textbf{1} &
  \textbf{2-5} &
  \textbf{6-9} &
  \textbf{10-14} &
  \textbf{$\geq$15} &
  \textbf{1} &
  \textbf{2-5} &
  \textbf{6-9} &
  \textbf{10-14} &
  \textbf{$\geq$15} \\ \hline
\begin{tabular}[c]{@{}l@{}}\% of truck driver advertisers who  \\ exclusively depict men as truck driver\end{tabular} &
  56 &
  79 &
  66 &
  63 &
  60 &
  24 &
  72 &
  73 &
  50 &
  40 &
  14 \\
\begin{tabular}[c]{@{}l@{}}\% of nurses advertisers who  \\ exclusively depict women as nurses\end{tabular} &
  46 &
  73 &
  48 &
  30 &
  40 &
  18 &
  69 &
  49 &
  29 &
  35 &
  5 \\ \hline
\end{tabular}}
\end{table}
